LightGen: Efficient Image Generation through Knowledge Distillation and Direct Preference Optimization

Recent advances in text-to-image generation have primarily relied on extensive datasets and parameter-heavy architectures. These requirements severely limit accessibility for researchers and practitioners who lack substantial computational resources. In this paper, we introduce \model, an efficient training paradigm for image generation models that uses knowledge distillation (KD) and Direct Preference Optimization (DPO). Drawing inspiration from the success of data KD techniques widely adopted in Multi-Modal Large Language Models (MLLMs), LightGen distills knowledge from state-of-the-art (SOTA) text-to-image models into a compact Masked Autoregressive (MAR) architecture with only $0.7B$ parameters. Using a compact synthetic dataset of just $2M$ high-quality images generated from varied captions, we demonstrate that data diversity significantly outweighs data volume in determining model performance. This strategy dramatically reduces computational demands and reduces pre-training time from potentially thousands of GPU-days to merely 88 GPU-days. Furthermore, to address the inherent shortcomings of synthetic data, particularly poor high-frequency details and spatial inaccuracies, we integrate the DPO technique that refines image fidelity and positional accuracy. Comprehensive experiments confirm that LightGen achieves image generation quality comparable to SOTA models while significantly reducing computational resources and expanding accessibility for resource-constrained environments. Code is available at https://github.com/XianfengWu01/LightGen

==> sec/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}

% Many researchers have recently focused on the visual generative model because different generative models can solve many tasks such as image generation~\cite{xiao2024omnigen, fan2025scaling, Rombach_2022_CVPR, flux2024}, image editing~\cite{lin2024text, feng2024dit4editdiffusiontransformerimage, wang2024tamingrectifiedflowinversion}, video generation~\cite{zheng2024opensorademocratizingefficientvideo, lin2024opensoraplanopensourcelarge, yang2024cogvideox}, video editing, etc. But it is very hard for us to get a good generative model, many generative models use many images in the pre-training stage, and it cost too much time and resource. It may have many redundant images for generative model to pre-train, so we want to provide a pre-train method that it does not need large GPU resource and many private data to pre-train. It will only use an open source dataset to pretrain, then post-process via DPO. It will achieve a capability comparable to that of SOTA to generate good quality. 

% The field of generative AI has seen remarkable progress, with diffusion models and autoregressive architectures leading the way in image generation and editing. While diffusion models excel at producing high-quality images, they often require significant computational resources and struggle with fine-grained editing tasks. On the other hand, autoregressive models offer precise control over image generation but can be computationally expensive to train and scale. Bridging these two paradigms to create a unified model capable of both tasks efficiently, without introducing additional modules, remains an open challenge.

% In this work, we propose a novel framework that leverages the strengths of masked autoregressive models and diffusion bridges to achieve efficient pre-training for image generation while simultaneously equipping the model with image editing capabilities. Our approach begins with a masked autoregressive model, which learns robust visual representations through efficient pre-training. By masking portions of the input and predicting the missing tokens, the model achieves high-quality image generation while minimizing computational costs. To enable image editing capabilities, we introduce a diffusion bridge model, which leverages the existing architecture to perform editing tasks without requiring new modules. This bridge allows the model to manipulate images with precision, such as object removal, style transfer, and content manipulation, while maintaining its generative performance.

% To further enhance the quality of the generated images, we apply post-processing techniques that refine the outputs of the model. These techniques improve the fidelity and realism of the generated images, ensuring that the model produces high-quality results without requiring extensive additional training or human feedback. This combination of efficient pre-training, diffusion bridges, and post-processing enables our framework to achieve state-of-the-art performance on both image generation and editing tasks.

% Our contributions are as follows:

% \item Masked Autoregressive Pre-training: We introduce a masked autoregressive model that learns rich visual representations efficiently, reducing computational costs compared to traditional methods.

% \item Diffusion Bridge for Editing: We propose a diffusion bridge that enables the model to perform image editing tasks without introducing new modules, leveraging the existing architecture.

% \item Post-processing for Quality Enhancement: We develop post-processing techniques that refine the outputs of the model, improving the quality of generated images.

% We evaluate our framework on a range of benchmarks, including text-to-image generation and image editing tasks, demonstrating its ability to achieve state-of-the-art performance while maintaining computational efficiency. Our results highlight the potential of combining masked autoregressive models with diffusion bridges for scalable and versatile visual content creation, offering a promising direction for future research in generative AI.

% The field of image generation has seen rapid advancements in recent years, with generative models such as Generative adversarial networks (GANs)~\cite{goodfellow2014gan}, Variational Autoencoders (VAEs)~\cite{kingma2013vae}, Flow-based models~\cite{Rezende2015pmlr}, Diffusion models~\cite{Rombach2022CVPR, Patrick2024ICML, flux2024, xiao2024omnigen} and autoregressive models~\cite{Li2024mar, fan2025scaling} achieving impressive results in tasks like image synthesis~\cite{Rombach2022CVPR}, super-resolution~\cite{Christian2017CVPR}, and inpainting~\cite{Yang_2017_CVPR}, etc. Diffusion Transformer models~\cite{William2023ICCV, Patrick2024ICML, flux2024} and Autoregressive models~\cite{Li2024mar, fan2025scaling} have demonstrated the ability to generate high-quality images from a variety of input conditions~\cite{Zhang_2023_ICCV, zhang2025scaling}, including text descriptions, sketches, lighting, and other forms of partial information. However, the success of these models often comes at the cost of significant computational resources and large-scale datasets~\cite{schuhmann2022laionb, chen2023pali}, which can be difficult or even impossible for many researchers to access.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1.0\linewidth]{ICCV2025-Author-Kit-Feb/fig/figure2_1.jpg}
%     % \includesvg[width=1.0\linewidth]{ICCV2025-Author-Kit-Feb/fig/figure2.svg}
%     \caption{In recent years, most image generation models have relied on large GPU clusters and private datasets for pre-training, making it difficult for most researchers to reproduce. This work addresses the challenge of reducing computational and dataset demands while achieving competitive results.}	
%     \label{fig:fig2}
% \end{figure}

% One of the primary challenges in generative modeling is the trade-off between performance and the resources required for training. SOTA models, particularly in the text-to-image domain, typically require large amounts of labeled data (often on the scale of $\mathcal{O}(100M)$ to $\mathcal{O}(1B)$ images) and extensive pre-training on high-performance GPU clusters. These resource demands make it difficult for smaller research teams or independent developers to reproduce or extend these models, limiting the accessibility of cutting-edge generative techniques.

% In this work, we propose a novel approach for efficient pre-training that significantly reduces both the dataset size and computational costs, without sacrificing performance. Our method leverages a much smaller open-source dataset of only $\mathcal{O}(1M)$ images, such as label-to-image datasets, without requiring complex data filtering, compared to the large $\mathcal{O}(100M)$ datasets used by existing text-to-image models. By reduce both the data required and the number of pre-training steps (to less than $\frac{1}{10}$ of traditional methods), we reduce the overall pre-training time and GPU resource usage, making high-performance image generation more accessible. By pre-training on an artifact dataset, which contains high-quality generated images, our model is able to achieve competitive performance at a $256px$ resolution on established benchmarks (e.g., GeneVal~\cite{ghosh2023geneval}). However, while $256px$ results are impressive, they still fall short compared to high-resolution generators. To bridge this gap, we subsequently fine-tune our model on $512px$ images. 

% It is important to note that pre-training on a high-quality artifact dataset combined with our preprocessing approach can introduce challenges, such as a lack of high-frequency details and difficulties in generating accurate positional information. To overcome these limitations, we incorporate a post-processing technique called Direct Preference Optimization (DPO)~\cite{rafailov2023direct}. DPO refines the generator by enhancing image quality and incorporating positional signals, thereby mitigating issues associated with the initial pre-training and preprocessing stages, ensuring that our model remains competitive with SOTA models, despite the significantly reduced training costs.

% Our approach, therefore, not only drastically reduces the amount of data and computational resources required but also accelerates the training process for text-to-image tasks. The experimental results demonstrate that our method achieves performance comparable to SOTA image generation models while significantly lowering resource demands and training time.

% Our contributions are as follows:

% \begin{itemize} 
% \item \textbf{Masked Autoregressive Pre-training:} We propose an efficient pre-training method for masked autoregressive models that significantly reduces dataset size and pre-training steps without architecture modified, ensuring competitive performance.
% \item \textbf{Post-processing for Quality Enhancement:} We introduce Direct Preference Optimization (DPO) as a post-processing technique to further enhance the quality of generated images by addressing issues such as loss of high-frequency details and positional inaccuracies.
% \end{itemize}

% The remainder of this paper is organized as follows: Section 2 provides a review of related work in generative modeling and the challenges associated with data and resource requirements. Section 3 presents the preliminary aspects of this work. In Section 4, we describe the details of our proposed method, including model architecture and the efficient pre-training and post-processing strategies. Section 5 presents experimental results and comparisons with existing methods. Finally, Section 6 concludes the paper and outlines future directions for further optimization and exploration.


The field of image generation has seen rapid advancements in recent years, with generative models such as Generative Adversarial Networks (GANs)~\cite{goodfellow2014gan}, Variational Autoencoders (VAEs)~\cite{kingma2013vae}, flow-based models~\cite{Rezende2015pmlr}, diffusion models~\cite{Rombach2022CVPR, Patrick2024ICML, flux2024, xiao2024omnigen}, and autoregressive models~\cite{Li2024mar, fan2025scaling} achieving impressive results in tasks such as image synthesis~\cite{Rombach2022CVPR, dhariwal2021diffusion}, super-resolution~\cite{Christian2017CVPR}, and inpainting~\cite{Yang_2017_CVPR}. Moreover, Diffusion Transformer models~\cite{William2023ICCV, Patrick2024ICML, flux2024} and autoregressive models~\cite{Li2024mar, fan2025scaling} have demonstrated the ability to generate high-quality images from a wide range of input conditions—including text descriptions, sketches, and lighting cues. However, the success of these models often comes at the cost of significant computational resources and large-scale datasets~\cite{schuhmann2022laionb, chen2023pali}, which can be prohibitive for many researchers.

One of the primary challenges in generative modeling is the trade-off between performance and the resources required for training. SOTA models, particularly in the text-to-image domain, typically require vast amounts of labeled data (often on the scale of $\mathcal{O}(100M)$ to $\mathcal{O}(1B)$ images) and extensive pre-training on high-performance GPU clusters. These resource demands limit the accessibility of cutting-edge generative techniques for smaller research teams and independent developers.

In this work, we propose a novel approach for efficient pre-training that significantly reduces both the dataset size and computational costs without sacrificing performance in a \textbf{small autoregressive model}. Our method leverages a much smaller open-source dataset~\cite{zk2024text2img} of \textbf{only $\mathcal{O}(1M)$ images}. This dataset contains high-quality image data generated by SOTA models such as \textbf{Flux}~\cite{flux2024} and \textbf{DALLE3}~\cite{openai2023dalle3}, and is of the same order of magnitude as typical label-to-image datasets~\cite{Jia2009imagenet}. By learning the features from these high-quality generated images, our model rapidly acquires strong generative capabilities, eliminating the need for complex data filtering used in large-scale datasets. Moreover, by reducing both the amount of data and the number of pre-training steps (to less than $\frac{1}{10}$ of traditional methods), we drastically decrease overall pre-training time and GPU resource usage, making high-performance image generation more accessible.

Pre-training is performed on an artifact dataset composed of high-quality generated images, enabling our model to achieve competitive performance at a $256 \times 256$ resolution on established benchmarks (e.g., GenEval~\cite{ghosh2023geneval}). However, while the $256 \times 256$ results are impressive, they still fall short of what high-resolution generators can achieve. To bridge this gap, we subsequently fine-tune our model on $512 \times 512$ images using the same dataset.

It is important to note that pre-training on a high-quality artifact dataset, combined with our preprocessing approach, can introduce challenges such as a lack of high-frequency details and difficulties in generating accurate positional information. To overcome these limitations, we incorporate a post-processing technique called Direct Preference Optimization (DPO)~\cite{rafailov2023direct}. DPO refines the generator by enhancing image quality and incorporating positional signals, thereby mitigating issues associated with the initial pre-training and preprocessing stages while ensuring that our model remains competitive with SOTA approaches, despite the significantly reduced training costs.

Our approach not only drastically reduces the amount of data and computational resources required but also accelerates the training process for text-to-image tasks. Experimental results demonstrate that our method achieves performance comparable to SOTA image generation models while significantly lowering resource demands and training time.

Our contributions are as follows:
% \begin{itemize} 
%     \item \textbf{Masked Autoregressive Pre-training:} We propose an efficient pre-training method for masked autoregressive models that significantly reduces dataset size and pre-training steps without modifying the architecture, ensuring competitive performance.
%     \item \textbf{Post-processing for Quality Enhancement:} We introduce Direct Preference Optimization (DPO) as a post-processing technique to further enhance the quality of generated images by addressing issues such as the loss of high-frequency details and positional inaccuracies.
% \end{itemize}
\begin{itemize}
    \item \textbf{Masked Autoregressive Pre-training Pipeline:} We propose an efficient masked autoregressive pre-training strategy that leverages high-quality generated data rapidly to achieve comparable generative performance without architectural modifications.
    \item \textbf{Fewer Parameter :} By maintaining less than $\tfrac{1}{10}$ the parameter size of SOTA models, we achieve comparable results while substantially reducing computational overhead.
    \item \textbf{Fast Training with Small Datasets:} Our approach accelerates training by relying on a smaller dataset (\textbf{only $\mathcal{O}(1M)$ images}) and fewer parameters, drastically cutting down on both training time and GPU usage.
    \item \textbf{Post-processing for Quality Enhancement:} We introduce Direct Preference Optimization (DPO) as a post-processing technique to address issues such as the loss of high-frequency details and positional inaccuracies, enabling our model to achieve or even surpass state-of-the-art quality.
\end{itemize}

The remainder of this paper is organized as follows: Section 2 reviews related work in generative modeling and the challenges associated with large-scale data and resource requirements. Section 3 presents the preliminary concepts underlying our approach. In Section 4, we detail our proposed method, including the model architecture and our efficient pre-training and post-processing strategies. Section 5 presents experimental results and comparisons with existing methods. Finally, Section 6 concludes the paper and outlines future directions for further optimization and exploration.


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
